Beyond Patents: R&D, Capital, and the Productivity Puzzle in Early-Stage High-Tech Firms

This study investigates the relationship between innovation activities and firm-level productivity among early-stage high-tech startups in China. Using a proprietary dataset encompassing patent records, R&D expenditures, capital valuation, and firm performance from 2020 to 2024, we examine whether and how innovation, measured by patents and R&D input, translates into economic output. Contrary to established literature, we find that patent output does not significantly contribute to either income or profit among the sampled firms. Further investigation reveals that patents may primarily serve a signaling function to external investors and policymakers, rather than reflecting true innovative productivity. In contrast, R&D expenditure shows a consistent and positive association with firm performance. Through mechanism analysis, we explore three channels (organizational environment, employee quality, and policy-driven incentives) to explain the impact of R&D, identifying capital inflow and valuation as key drivers of R&D investment. Finally, heterogeneity analysis indicates that the effects of R&D are more pronounced in sub-industries such as smart terminals and digital creativity, and for firms based in Shenzhen. Our findings challenge the prevailing assumption that patent output is a universal indicator of innovation success and underscore the context-dependent nature of innovation-performance linkages in emerging markets.

==> firm_reg_year.tex <==
reg\_year&Number&Percentage \\
\hline
2000&1&\$0.2 \\
2003&1&\$0.2 \\
2010&1&\$0.2 \\
2011&1&\$0.2 \\
2012&1&\$0.2 \\
2014&5&\$0.8 \\
2015&8&\$1.3 \\
2016&23&\$3.7 \\
2017&56&\$8.9 \\
2018&98&\$15.6 \\
2019&83&\$13.2 \\
2020&110&\$17.5 \\
2021&129&\$20.5 \\
2022&56&\$8.9 \\
2023&37&\$5.9 \\
2024&16&\$2.5 \\
2025&2&\$0.3 \\
Total&628&\$100.0 \\


==> relation_patent_Capitial_new2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{2025 Patents Num.}&\multicolumn{1}{c}{2025 Patents Num.}&\multicolumn{1}{c}{2025 Patents Num.}\\
[0.5em]
\hline
R\&D Expenditure in 2024&      0.0760         &      0.0885         &     -0.0632         \\
                    &     (0.365)         &     (0.359)         &     (0.388)         \\
[1em]
Valuations&       1.060         &       1.006         &       1.413\sym{*}  \\
                    &     (0.702)         &     (0.711)         &     (0.833)         \\
[1em]
Investment Rounds&       1.181         &       1.110         &       0.491         \\
                    &     (0.766)         &     (0.767)         &     (0.852)         \\
[1em]
Employee Numbers   &      0.0484\sym{***}&      0.0487\sym{***}&      0.0555\sym{***}\\
                    &    (0.0126)         &    (0.0127)         &    (0.0125)         \\
[1em]
Industry FE &  & \checkmark & \checkmark \\
[1em]
Year FE     &  &  & \checkmark \\
[1em]
Stage FE    &  &  & \checkmark \\
[1em]
SZ Indicator &  &  & \checkmark \\
[1em]
\hline
Observations        &         323         &         323         &         267         \\
[0.5em]
R-squared           &       0.237         &       0.275         &       0.390         \\
\hline\hline
\end{tabular}
}

